Combined D0 Measurements Constraining the CP-violating Phase and Width Difference in the $B_s^0$ System

We combine the D0 measurement of the width difference between the light and heavy B_s^0 mass eigenstates and of the CP-violating mixing phase determined from the time-dependent angular distributions in the B_s -> J/psi phi decays along with the charge asymmetry in semileptonic decays also measured with the D0 detector. With the additional constraint from the world average of the flavor-specific B_s^0 lifetime, we obtain Delta Gamma_s = (\Gamma_L - \Gamma_H) = 0.13 +- 0.09 ps$^{-1}$ and phi_s = -0.70 ^{+0.47}_{-0.39}. The data sample corresponds to an integrated luminosity of 1.1 fb^{-1} accumulated with the D0 detector at the Fermilab Tevatron Collider.

==> list_of_visitor_addresses_r2.tex <==
% list_of_visitor_addresses_r2.tex                            1/5/07
%
%
\bibitem[*]{alton}
Visitor from Augustana College, Sioux Falls, SD, USA
\bibitem[\S]{podesta-lerma}
Visitor from ICN-UNAM, Mexico City, Mexico.
%\bibitem[\dag]{kozminski}
%Visitor from Lewis University, Romeoville, IL, USA
\bibitem[\ddag]{voutilainen}
Visitor from Helsinki Institute of Physics, Helsinki, Finland.
\bibitem[\#]{wenger}
Visitor from Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland.
%
\vskip 0.25cm

